WaveGlow: A Flow-based Generative Network for Speech Synthesis

In this paper we propose WaveGlow: a flow-based network capable of generating high quality speech from mel-spectrograms. WaveGlow combines insights from Glow and WaveNet in order to provide fast, efficient and high-quality audio synthesis, without the need for auto-regression. WaveGlow is implemented using only a single network, trained using only a single cost function: maximizing the likelihood of the training data, which makes the training procedure simple and stable. Our PyTorch implementation produces audio samples at a rate of more than 500 kHz on an NVIDIA V100 GPU. Mean Opinion Scores show that it delivers audio quality as good as the best publicly available WaveNet implementation. All code will be made publicly available online.

==> fig_fp16_rtperf.tex <==
%auto-ignore
\begin{figure}
\begin{tikzpicture}
\begin{axis}[
    title={WaveGlow FP16 Inference Performance},
    xlabel={Number of voices},
    ylabel={Real time factor},
    xmin=0, xmax=10,
    ymin=0, ymax=26,
    xtick={1, 2, 4, 8},
    ytick={3,6,12,20,25},
    legend pos=north east,
    ymajorgrids=true,
    grid style=dashed,
]

\newcommand\framesastime{88/(22050/256)}
\addplot[
    color=red,
    mark=square,
    ]
    coordinates {
    (1,\framesastime/0.1827068328857422)
    (2,\framesastime/0.17424988746643066)
    (4,\framesastime/0.205582857131958)
    (8,\framesastime/0.3236267566680908)
    };
    \addlegendentry{1 second}

\addplot[
    color=green,
    mark=square,
    ]
    coordinates {
    (1,2*\framesastime/0.16884613037109375)
    (2,2*\framesastime/0.19608139991760254)
    (4,2*\framesastime/0.3258688449859619)
    };
    \addlegendentry{2 seconds}


\addplot[
    color=blue,
    mark=square,
    ]
    coordinates {
    (1,4*\framesastime/0.17935514450073242)
    (2,4*\framesastime/0.3257107734680176)
    };
    \addlegendentry{4 seconds}
    
\addplot[
    color=black,
    mark=square,
    ]
    coordinates {
    (1,8*\framesastime/0.3265964984893799)
    };
    \addlegendentry{8 seconds}
    
    
\end{axis}  
\end{tikzpicture}
\caption{WaveGlow FP16 Real-time inference speed given number of voices on a single V100 NVIDIA GPU.} \label{fig:fp16_rtperf}
\end{figure}
